LiCo-Net: Linearized Convolution Network for Hardware-efficient Keyword Spotting

This paper proposes a hardware-efficient architecture, Linearized Convolution Network (LiCo-Net) for keyword spotting. It is optimized specifically for low-power processor units like microcontrollers. ML operators exhibit heterogeneous efficiency profiles on power-efficient hardware. Given the exact theoretical computation cost, int8 operators are more computation-effective than float operators, and linear layers are often more efficient than other layers. The proposed LiCo-Net is a dual-phase system that uses the efficient int8 linear operators at the inference phase and applies streaming convolutions at the training phase to maintain a high model capacity. The experimental results show that LiCo-Net outperforms single-value decomposition filter (SVDF) on hardware efficiency with on-par detection performance. Compared to SVDF, LiCo-Net reduces cycles by 40% on HiFi4 DSP.

==> icassp/priorworks.tex <==
% \section{Prior Works}\label{sec:priorworks}

% Some past work explores the idea of sparse supernet for ASR model training. Wu et. al.~\cite{wu2021dynamic} developed dynamic sparsity for neural-network (DSNN) based speech models, as a framework to train a few speech models at pre-defined sparsity in one supernet. Different from our work, the DSNN applies a fixed number of pre-defined target sparsity level uniformly to each of the layers of the ASR models. It can not produce model with sparsity not pre-defined in the training process. In addition, it is not guaranteed that the DSNN-trained models would lie on the Pareto front of WER vs model size.

% Other works apply differentiable architecture search (Darts)~\cite{liu2019darts} to ASR models~\cite{liu2021improved, hu2021neural, shi2021dartsconformer} or end-to-end key word spotting models~\cite{zhang2020autokws}. In general, these work differ from our work in that they focus on varying layer operation type, layer width and sizes. 
% In~\cite{liu2021improved,shi2021dartsconformer}, the authors used Darts to search for different combinations of convolution, feed-forward network and multi-headed self attention blocks inside the conformation modules. Their work do not address model compression and the trade off between WER and model sizes. In addition, the Darts-based NAS utilizes validation loss, instead of the final model evaluation metrics (i.e. WER), to determine optimal architecture. 
